Skyeye Team at MBZIRC 2020: A team of aerial and ground robots for GPS-denied autonomous fire extinguishing in an urban building scenario

The paper presents a framework for fire extinguishing in an urban scenario by a team of aerial and ground robots. The system was developed to address Challenge 3 of the 2020Mohamed Bin Zayed International Robotics Challenge (MBZIRC). The challenge required to autonomously detect, locate and extinguish fires on different floors of a building, as well as in its surroundings. The multi-robot system developed consists of a heterogeneous robot team of up to three Unmanned Aerial Vehicles (UAV) and one Unmanned Ground Vehicle (UGV). We describe the main hardware and software components for UAV and UGVplatforms and also present the main algorithmic components of the system: a 3D LIDAR-based mapping and localization module able to work in GPS-denied scenarios; a global planner and a fast local re-planning system for robot navigation; infrared-based perception and robot actuation control for fire extinguishing; and a mission executive and coordination module based on Behavior Trees. The paper finally describes the results obtained during the competition, where the system worked fully autonomously and scored in all the trials performed. The presented system ended in 7th position out of 20 teams in the Challenge3 competition and in 5th position (out of 17 teams) in the Challenge 3 entry to the Grand Finale (Grand Challenge) of MBZIRC 2020 competition.

==> 08_LessonsLearn.tex <==
This section analyzes the performance of our system and the lessons we learned during the MBZIRC 2020 competition. We certainly learned some lessons throughout the development process prior to the competition and during the actual competition.

\subsection{Hardware}
In this part, our learning is mainly related to the performance of the fire extinguishing system. First of all, in the case of UAVs, the system is light and equally balanced, therefore, it has advantages in terms of maneuverability and stability. This allowed the drone to be located at the point of attack on the fire with precision. Secondly, despite the fact that having a water ejection system with success on the target, our proposed approach %to the blocking zone 
does not provide feedback on the ejection. To overcome it,the system can be improved by including a high-pressure ejection system%, which gives us certainty that the water follows a straight line for a few meters, 
,or else to include a visual system to control in closed-loop the water path. Third, in the case of the deployment of the blanket,%, despite the fact that the drone found and was located over the fire, the subsequent maneuvers were not sufficient for the blanket 
the blanket failed on covering the whole target, due to the air turbulence generated by the own UAV. Therefore, an approach to improve the system is to let to fall in a straight line, and to decrease the distance on which the deployment is carried out.% the blanket a short distance of reaching the objective.
Finally, the UGV would benefit on a height increase of its extinguishing mechanism. This would avoiding the chance of an obstacle ocluding the fire and would increase the chance of hitting the target when detected.%with respect to the UGV, despite the fact that the system had great robustness to detect fire, being a low-height platform,  in the path of the water, more than once occlusion was generated, thus, including units that allow a greater scope and approach to the objective, would improve the chances of success.

%Another important aspect to consider is the performance of the 3D OS-1-16 LIDAR. This made it possible to obtain a high resolution map, especially in the outdoor part of the stage given the greater aperture of the laser, detected objects, such as safety nets. Consequently, the recreation of the real scene with such a level of detail contributed to having a robust location independent of the GPS. DAvid: esto se repite en la parte de Localization

\subsection{Localization}

The location achieved during the competition had a stable performance and a good precision without the use of GPS, relying only on the use of LIDAR measures that were matched against a 3D map obtained a priori. Thus, the combination of LOAM for robot odometry and MCL3D for long-term localization seems to be good choice for UAVs. This approach allowed us for fast system deployment, as we do not need to wait for GPS fix. Most importantly, this made the indoor-outdoor transition on localization seamless. It also was very important in order to be able to safely navigate in the scenario, as the localization of our platforms was performed taking into account the different elements on the stage, e.g. columns or safety nets, allowing us to locate them with good precision against the obstacles in the environment. Last but not least, other teams experienced localization issues when relying on GPS due to signal degradation. Also, 

Nevertheless, relying in a non-GPS approach has its risks. We experienced some localization issues on the UGV platform in the Grand Challenge due an incorrect initialization of the MCL. As there were not enough features in the environment, the system could not make  corrections and converge to the actual position on time. Thus, the user should be very careful in the initialization of the platform to prevent such issues. Finally, we also detected an increase in the localization error when robots performed maneuvers with high yaw rate when using LIDAR-based odometry. To handle this, we limited the maximum turn rate of the platforms which used it. 

\subsection{Mission Execution}

The BT-based mission execution proposed in this paper has demonstrated its potential to specify simple missions involving multiple systems. It has enough features to specify most of the required conditions for the execution of a mobile robot interacting with the environment. Also, the visual tool for BT specification and state visualization really helps for debugging and mission specification. The only room for improvement here is to develop a GUI tool for precise waypoint specification and for increasing productivity.  %  parameter tuning??

%However, the specification of the mission was still complex because most of the goals and actions were dependant on the actual map used for localization. Moreover, we had to specified the actual coordinates on a separate file, making it more difficult to debug. Robot way-point must be specified in the world system reference, and it is sometimes difficult to understand which is the best position/orientation to monitor targets in the environment. Thus, a GUI tool for goal and way-point definition using the actual map would significantly simplify the mission specification.



==> 09_Conclusion.tex <==
%In this work, the hardware and software systems that are implemented as the proposed strategies to solve Challenge 1 and Challenge 3 of the 2020 Mohamed Bin Zayed International Robotics Challenge (MBZIRC) have been detailed. The contributions presented have been developed by the Skyeye team, a consortium of research groups from the Universidad Polit\'ecnica de Madrid and the Universidad Pablo Olavide. The 2020 MBZIRC challenges present complex environments and scenarios, which must be completed using fully autonomous robotic systems. As such, a diverse knowledge of various fields is necessary to implement efficient and robust solutions.

%The aim of challenge 1 will be to test the capabilities of autonomous UAV systems for detection and interaction with static and dynamic objects. The results obtained from the experimental tests demonstrate the functionality and validity of the overall strategy proposed for challenge 1. In these tests, a UAV platform was able to autonomously execute complex tasks in outdoor conditions to locate, follow and retrieve an object tethered to a target UAV in flight. Nevertheless, given that the overall system is primarily based on computer vision techniques, several complication can arise when extremely varying lighting conditions are present. Moreover, the objective of Challenge 3 is to use several robots (ground and aerial platforms) to extinguish fires in an urban-like scenario. The preliminary experiments have been presented showing the main functionalities of the system, such as mapping, localization, navigation, fire detection and extinguish, including integrated full missions from the individual vehicles. 

%The future work to be performed entails the continuation of the flight tests to explore the most outdoor scenarios that could possibly be found in challenge 1. Additionally, the challenge 3 work will focus on the coordination between ground and aerial vehicles, and performing final experiments on the indoor navigation of the UAVs in a scenario built to replicate the real environment to be found at the final event before attending the MBZIRC competition February 20-25 at the Abu Dhabi National Exhibition Center in Abu Dhabi, (UAE). 

We present in this article a cooperative multi-robot team framework approach to tackle MBZIRC Challenge 3: ``Team of Robots to FightFire in High Rise Building". This Challenge takes place in an open-air arena with a building in the middle, and consists of searching, detecting and extinguishing fires located on the ground, exterior walls of the building and in the different interior levels of the building.

The paper describes the design parts that we consider as the most significant factors leading to the best performance of the system in the competition. First, the system is able to coordinate missions for multiple robots using behavior tree. Second, each robot is able to following waypoints and avoid obstacles to success in the navigation tasks. Third, each robot with its corresponding sensors on board, are able to locate itself with great precision and stability throughout the course of the competition, based on the use of LOAM and 3D MCL modules.
Fourth, each of the robots for the different deployment areas (e.g. inside the building, walls of the building, outdoor part of arena), has modules to searching, detecting and locating the fire, which were executed during the competition, proving their functionality. The only modules that were not tested in the competition,  are the one to execute in the upper floors of the building since our UAVs did not enter into the buildings due to time constraints %it was not possible to enter these floors
. However, they were tested in simulation. Finally, it was proven that each of the robots is capable of attacking the fire for which it was prepared once a fire is detected. In the case of the M600 and M210, ejecting water to the walls of the building, and also, only in the case of the M600, deploying a blanket over the fires on the outdoor ground. As for the UGV (SIAR), ejecting water. Something important in this last point is that the extinguishing system, which attacks the fire, can be considerably improved, in such a way as to increase the probability of success in the extinguishing task, which is considered as future work.

The above is reflected in the results shown in the experiments and results section, as well as in the multimedia material described that shows the performance of the multi-robot framework. However, the most meaningful and credible verification of the performance and the reliability of the system was achieved in the MBZIRC competition the 7th place in Challenge 3 among 20 teams, and the 3rd place in the Grand Challenge among 17 teams.

Our main motivation to present the development of this multi-robot team framework is the contribution in the state-of-the-art in robotics, which could facilitate the deployment of multi-robot autonomous platforms in real and dangerous scenarios, motivated by the needs to approach the fire disasters in a faster way and reducing the risk of humans that work on these conditions.







==> SoftwareArchitecture.tex <==
The implemented software architecture provides the functionalities required for autonomous navigation of each robot in an urban firefighting scenario and makes use of the robot platforms and sensors described in \ref{hardware}, to develop these functionalities (self-localization, navigation, inspections, etc). Figure \ref{fig:soft_archi} shows the software architecture proposed. This architecture relies on the framework Robot Operating System \cite{Quigley09}, using the ros-kinetic distribution under Ubuntu 16.04. 

The framework used for the mission execution and monitoring of heterogeneous robots is based on Beharviour Trees (BTs). The main idea to accomplish the mission is to check all the points where there could be a fire in the scenario. That points are given through a waypoints route from the mission. Once the robot reaches a waypoint, a searching maneuver is done in order to detect fire (see \ref{subsec:extinguish}). In case of finding a fire, the centering-extinguishing task is launched. Otherwise the robot continues to next way-point.

The navigation along the path defined by the set of way-points is performed by using the IMU and LIDAR measurements. Thus, global planner and local planner generate the trajectories to track the way-points. Both global and local planner receive the robot localization and map of the environment for generating the corresponding trajectories.

To sequence the task of: searching, detecting and centering fire, we use in these modules the ROS library ``actionlib". Thus, once the robot reaches a way-point, a goal is sent to start the searching fire task, if during this task the fire is detected, the ``actionlib" sends a success and the centering task begins, and thus, once centered, the extinguishing task is executed, ejecting water or drooping the blanket. Figure \ref{fig:diagram_fire_detection} shows the fire perception and extinguishing system.

\begin{figure}[t]
	\centering
    \includegraphics[width = 1\textwidth]{Figures/Soft_Architecture.jpg}
	\caption{Software architecture of the Fire Extinguishing System.}
	\label{fig:soft_archi}
\end{figure}



% The modules developed are common for UGVs and UAVs.

% \begin{itemize}

% \item \textbf{Odometry}: It provides LIDAR-based odometry estimates by fusing IMU and 3D Lidar. In this way, the robots platform are able to precisely and robustly estimate a 6-DOF odometry.

% \item \textbf{3D mapping}: It gets the enhanced odometry outputs and uses them to integrate the measurements from the  3D LIDAR. This allows a precise 3D reconstructions of scenery in real-time. 

% \item \textbf{Localization}: A 3D approach is used as a localization module which is based on Monte Carlo localization (MCL). This module provides a robust global position. 

% \item \textbf{Navigation}: This module offers the capability to safely navigate in a mode fully autonomous avoiding obstacles, following way points, and executing rotation in place maneuvers in case of narrow places. 
% %This module is based on Theta Lazy* Planner to get a global and local path. The planner reaches a collision free path with minimum distance between point, which allows moving as fast as possible through the scenery and generates a sequence of commands that allow the robot to safely cross the path\cite{etfa19arco}. 

% \item \textbf{Fire perception and extinguishing}: This module process the information from the thermal camera to detect fire. Once the fire is detected, robot is approached to extinguishing through spray water or drop blanket.

% \item \textbf{Executive Layer}: It is the highest software layer developed and is in charge to manage the information of the previous modules and coordinate tasks that are performed in the firefighting scenario to extinguish the fires.

% \end{itemize}
 
% \subsubsection{Unmanned ground vehicle}

% These modules developed for the UGV are the following:

% \begin{itemize}

% \item \textbf{SIAR driver}: Software that interfaces with the hardware board of the robot, and offers a standard ROS commands and services for easy integration of the robot with the rest of the system. 

% \item \textbf{IMU driver}: This filters the raw data produced by the inexpensive IMU sensor Arduimu v3.

% \end{itemize}

% \subsubsection{Unmanned aerial vehicle}

% These modules developed for the UAV are the following:

% \begin{itemize}

% \item \textbf{UAV driver}: 


% \end{itemize}

==> Team.tex <==
The Challenge 3 requires a team of UAVs and UGV collaborating in order to autonomously extinguish a series of simulated fires in an urban high rise building firefighting scenario. The objective is to carry out a series of urban firefighting related tasks in an outdoor-indoor environment. The robots has to extinguish a set of fires using water, including fires inside the building and located in its facade. Furthermore, fires located at ground level outside the building must be extinguished using fire blankets carried by the robots. Figure \ref{fig:arena} shows the arena.

\begin{figure}[ht]
	\centering
    \includegraphics[width =0.7\textwidth]{Figures/arena.jpg}
	\caption{Arena of the Challenge 3.}
	\label{fig:arena}
\end{figure}

The technological challenges addressed include, fast autonomous navigation in semi-unstructured, complex, dynamic environments, with reduced visibility (e.g. smoke) and minimal prior knowledge, robust perception, sensing and avoiding obstacles, GPS denied navigation in indoor-outdoor environments, physical interactions, and air-surface collaboration.

Both UAV and UGV are equipped with a water tank and a set of water pumps to extinguish the fires. The speed of the UAVs is restricted to a maximum of 30 km/hour and the speed of the UGV is restricted to a maximum of 15 km/hour. The size of the UAVs is restricted to a maximum volume of 1.2mx1.2mx0.5m, although a volume of 1.7mx1.7mx1m is also allowed but a penalty is applied in this case. The size of the UGVs is restricted to a maximum volume of 1.7mx1.5mx2m. The size of the area is approximately the size of half a football pitch and  contains a tall indoor structure simulating a high-rise building (See Figure XX). The duration of Challenge 3 is 15 minutes and of the Grand Challenge 25 minutes. The Grand Challenge is to compete in a triathlon type event combining the tree challenges. The Skyeye team participated in the Grand Challenge and we competed in the Challenge 3 described.

The organizers provided a standard control network across the arenas. Thus, the communication between UAVs and UGV is allowed. The network was setup as follows: Multi-channel, 20MHz and 5GHz, the latter supporting standards 802.11a, 802.11an and 802.11ac 

The fires are simulated at various locations at ground level in the arena and at different heights of the building (in the range of 5m to 15m). Figure \ref{fig:fires} shows both fires located in the facade, located at ground and inside the building in the ground floor.

\begin{figure}[ht]
	\centering
    \includegraphics[width = 0.47\textwidth]{Figures/fires_facade_ground.jpg}
    \includegraphics[width = 0.47\textwidth]{Figures/fire_ground_floor.jpg}
	\caption{Types of fires in the Challenge 3.}
	\label{fig:fires}
\end{figure}

The challenge has a number of separate tasks depending on the type of fire, so each task is scored separately. The score is got from the amount of water delivered in the fire of the building. The 100\% of score is obtained if the amount of water is 1 liter. The score of the ground fire is got by using fire blankets and it depends on the area covered by the blanket. The mission can be attempted in either full autonomous or manual mode and a lower score is obtained if the execution is not completed fully autonomously but with human intervention because any human intervention during the mission means that it is performed in manual mode. RTK/DGPS can be use although a penalty of 25\% will be applied if it is used. The team obtaining the highest score is the winner.

To accomplish the mission, we use a team of up to 2 UAVs and 1 UGV. Next sections describe the work team and proposed robotic team and their main modules. Then, we describe the cooperation in the team.  

\subsection{The robot team}

\subsubsection{Unmanned ground vehicle}
% David, review
The ground platform used for Challenge 3 is a 6-wheeled robot with indepenvamnd platform is (see Fig. \ref{fig:siar_sensors}):
\begin{itemize}
    \item Onboard computer: 5NUC5i7RYB.
    \item GPS sensor UBlox 8.
    \item IMU: ArduIMUv3.
    \item Infrared camera: A compact SeekThermal camera mounted on a pan\&tilt mechanism on top of the robot. The images are used for fire detection.
    \item 3D LIDAR: A 3D OS-1-16 LIDAR manufactured by Ouster has been installed on top of the robot. The information gathered by this sensor is used for localization and mapping.
    \item 2D LIDAR: A Hokuyo UTM-30LX sensor is installed. The information of this sensor is used for local obstacle detection/avoidance.
    \item Orbbec ASTRA camera. Used for providing the operator with images to allow remotely operating the platform. It is also used for indoor local obstacle avoidance.
\end{itemize}

\begin{figure}[ht]
	\centering
    \includegraphics[width = 0.47\textwidth]{Figures/siar_sensors_1.jpeg}
    \includegraphics[width = 0.47\textwidth]{Figures/siar_sensors_2.jpeg}
	\caption{Ground platform used for Challenge 3.}
	\label{fig:siar_sensors}
\end{figure}

\subsubsection{Unmanned aerial vehicles}
Regarding to the aerial platforms, the aerial robot models used for the competition will be adaptations of the DJI Matrice 210 V2 and the DJI Matrice 600 Pro. The aerial platforms are also equipped with a OS-1-16 LIDAR manufactured by Ouster, installed to the bottom of the robots. The LIDAR is able to provide 320k 3D points per second, ranging from 0.2 to 120 meters. The purpose of this sensor is threefold:
\begin{itemize}
    \item Environment mapping and odometry. This sensor is the basis for the generation of the 3D map of the environment. It is also used to compute an accurate robot odometry in the UAVs. 
    \item Robot localization. The 3D LIDAR is used as main sensor for robot localization in all robots, UAVs and UGV.
    \item Obstacle detection for robot navigation. The robot local planner uses this information to detect mid/long range obstacles (more than 2 meters) in order to properly react on time.
\end{itemize}

Fig. \ref{fig:m600} shows the DJI Matrice 600 Pro used for the preliminary experiments.

\begin{figure}[ht]
	\centering
    \includegraphics[width = 0.42\textwidth]{Figures/M600.jpeg}
    \includegraphics[width = 0.45\textwidth]{Figures/m600-building.jpg}
	\caption{DJI Matrice 600: one of the aerial platforms used for Challenge 3.}
	\label{fig:m600}
\end{figure}

==> annex_datatypes.tex <==
\section{Custom datatypes for SIAR platform}
\label{sec:custom_types}

Even though most of the information of the rosbag files presented in this paper uses standard types from the ROS base libraries, we opted to generate custom messages to group internal messages for introspective information of the SIAR platform. In this appendix, the information about our custom types is detailed.

\begin{itemize}
    \item s\texttt{iar\_driver/SiarStatus}. This topic contains information of the complete status of the platform. It includes information of the internal status of the platform, including raw odometry values, the status of width adjustment motors, the servos of the arm and the onboard lights. In addition, it provides information about the remaining battery and about the power supply, if connected. Below you can find the fields included in the topic:
    
    \footnotesize
    
    \begin{tabular}{lll}
         std\_msgs/Header header         & float32 electronics\_x         &    float64 x                                           \\
         string motor\_fw\_version       & float32 width                  &    float64 y                                           \\
         string battery\_fw\_version     & int64 front\_left\_ticks       &    float64 speed                                       \\
         int8 operation\_mode            & int64 front\_right\_ticks      &    siar\_driver/SiarBatteryMonitor elec\_battery       \\
         bool reverse                    & int64 middle\_left\_ticks      &    siar\_driver/SiarBatteryMonitor motor\_battery      \\
         bool slow                       & int64 middle\_right\_ticks     &    siar\_driver/SiarPowerSupply power\_supply          \\
         bool fan                        & int64 back\_left\_ticks        &    bool front\_light                                   \\          
         bool hard\_stop                 & int64 back\_right\_ticks       &    bool rear\_light                                    \\           
         bool is\_stopped                & int16[5] herculex\_position    &    uint8 aux\_pins\_values                             \\       
         uint8 hard\_stop\_time          & uint8[5] herculex\_temperature &    nav\_msgs/Odometry odom                             \\
         uint16 lin\_motor\_pos          & uint8[5] herculex\_status      &    bool arm\_panic    \\
         uint16 lin\_motor\_pot          & uint8[5] herculex\_torque      &    
    \end{tabular}
    
        
    \normalsize
    
    \item \texttt{siar\_driver/SiarBatteryMonitor}. This topic groups the information of the sensors for battery monitoring.
        
    \footnotesize
    
    \scalebox{0.9}{
    \begin{tabular}{p{0.25\textwidth}p{0.25\textwidth}p{0.4\textwidth}}
         float32 voltage &  float32 current   &   float32 integrated\_current \\  
         int8 percentage &  int16 remaining\_time & 
     \end{tabular}
     }
     
    \normalsize
    
    \item \texttt{rssi\_get/Nvip\_status}. This message has information about the communication link established between the onboard communication systems and the deployed communication systems.
    
    \footnotesize
    
    \begin{tabular}{p{0.25\textwidth}p{0.25\textwidth}p{0.25\textwidth}}
    %\begin{tabular}{l{4cm}l{4cm}l{4cm}}
         string mac &  int8 rssi\_perc   &   float32 rx\_rate \\  
         int8 rssi &  float32 tx\_rate & 
     \end{tabular}
    \normalsize
    \item \texttt{amcl\_sewer/Manhole}. This message has information related to the position of a detected manhole. It is used in the dataset to indicate the precise instant when the SIAR platform passed below a manhole. It can be used as partial ground truth to test localization systems.
    
    \footnotesize
    \scalebox{0.9}{
\begin{tabular}{p{0.15\textwidth}p{0.35\textwidth}p{0.4\textwidth}}
        int32 id &
         geometry\_msgs/Pose2D local\_position &
        nav\_msgs/NavSatFix gps\_position
    \end{tabular}
    }
      \normalsize
    \item 
\texttt{libelium\_waspmote\_gas\_node/GasMeasure}. Includes all the information related to one measurement of the gas sensor onboard the SIAR platform.
    
    \footnotesize
%     \scalebox{0.9}{
    
        \begin{tabular}{p{0.33\textwidth}p{0.33\textwidth}p{0.3\textwidth}}
        

std\_msgs/Header head &            float32 O2\_conc     &  bool O2\_alarm \\
int32 time &         float32 H2S\_conc    &  bool H2S\_alarm  \\
int8 bat\_perc &     float32 CO\_conc     &  bool CO\_alarm     \\
float32 bat\_level &   float32 CH4\_conc    &  bool CH4\_alarm   \\
float32 temperature & float32 pressure   &    float32 RH       \\
geometry\_msgs/Vector3 accel

\end{tabular}
    
%     }
    
\end{itemize}

